What You Really Need To Know About Your Neighbor

A fundamental question in system design is to decide how much of the design of one component must be known in order to successfully design another component of the system. We study this question in the setting of reactive synthesis, where one constructs a system implementation from a specification given in temporal logic. In previous work, we have shown that the system can be constructed compositionally, one component at a time, if the specification admits a "dominant" (as explained in Introduction) strategy for each component. In this paper, we generalize the approach to settings where dominant strategies only exist under certain assumptions about the future behavior of the other components. We present an incremental synthesis method based on the automatic construction of such assumptions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{21}
\providecommand{\publicationstatus}{Dimitrova, Piskac (Eds.): Fifth Workshop on\\ 
Synthesis (SYNT 2016)\\
EPTCS 229, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.229.4}{10.4204/EPTCS.229.4}}
\pdfoutput=1

